Weighted Tensor Decompositions for Context-aware Collaborative Filtering

Over recent years it has become well accepted that user interest is not static or immutable. There are a variety of contextual factors, such as time of day, the weather or the user's mood, that influence the current interests of the user. Modelling approaches need to take these factors into account if they want to succeed at finding the most relevant content to recommend given the situation. A popular method for context-aware recommendation is to encode context attributes as extra dimensions of the classic user-item interaction matrix, effectively turning it into a tensor, followed by applying the appropriate tensor decomposition methods to learn missing values. However, unlike with matrix factorization, where all decompositions are essentially a product of matrices, there exist many more options for decomposing tensors by combining vector, matrix and tensor products. We study the most successful decomposition methods that use weighted square loss and categorize them based on their tensor structure and regularization strategy. Additionally, we further extend the pool of methods by filling in the missing combinations. In this paper we provide an overview of the properties of the different decomposition methods, such as their complexity, scalability, and modelling capacity. These benefits are then contrasted with the performances achieved in offline experiments to gain more insight into which method to choose depending on a specific situation and constraints.

==> 02_related_work.tex <==
% !TeX root = WTF.tex

\section{Related Work}
\label{sec:rw}


% Tensor factorization
%  - CP
%  - HOSVD (similar to Tucker but orthogonal?)
%  - TTF
%  - PITF

\todonote{Tensor decomposition methods: CP, Tucker, TTF, PITF}


% Recommendation with Tensor factorization


WMF based tensor factorization~\cite{hidasi2012fast} (uses CP, method can use multiple dimensions, but only goes up to three).
Extension iTALSx with pairwise interaction model published later (2014)~\cite{hidasi2014factorization}. Seems like they stack context and limit it to 3 dimensions.
General framework published later (2016)~\cite{hidasi2016general}. Looks like a combination of CP and pairwise and maybe other interactions/weighting schemes. The best performing variant is found to be a model that has a component for user-item interaction plus components for context dependent 'offsets' (U I + USI + UQI). This is promising for our method.


\todonote{general paper about importance of context: \cite{pagano2016contextual}. They mention key challenges that need to be solved: Continuous context, missing values for context, scalability and evaluation.}


\todonote{2020 PITF paper. Seems like adaptation of iTALSx that does use multiple dimensions and uses some clever tricks to speed up computation. However doesn't scale well at all and only uses 10 factors which performs very bad in our experiments}

\todonote{multiverse recommendation (tucker, but only rating).}


%In factorization machines (FM), each element of an interaction (the user, item and context variables) is first binarised and stacked together in a binary vector $\bf x \in \R^{q}$. The model is of the form 
%$$ y( \bf x) = w_0 + \sum_{i = 1}^q w_i x_i + \sum_{i=1}^q \sum_{j = i+1}^q \bf (\bf v_i^T \bf v_j) \bf x_i \bf x_j $$
%where the vector $\bf v_i$ is the $i$th column of the matrix $\bf{V} \in \R^{k \times q}$. It is trained by real interactions (where the target value is $y = 1$) but also with false interactions (where the target value is $y = 0$). 
%Popular extensions on this model includes neural factorisation machines \cite{10.1145/3077136.3080777} and Field-Aware Factorisation machines (FFM).


\todonote{Touch on FM \cite{rendle2011fast} (also compares ALS with SGD) and extensions of FM: FFM, Gaussian processes~\cite{nguyen2014gaussian}}



%\todonote{Adversarial TF (RecSys2019)}
%\todonote{graph convolution machine (2021)}
%\todonote{Rating prediction: list}
%\todonote{CSLIM (2021) (rating only)}




